Differentiable Euler Characteristic Transforms for Shape Classification

The Euler Characteristic Transform (ECT) has proven to be a powerful representation, combining geometrical and topological characteristics of shapes and graphs. However, the ECT was hitherto unable to learn task-specific representations. We overcome this issue and develop a novel computational layer that enables learning the ECT in an end-to-end fashion. Our method, the Differentiable Euler Characteristic Transform (DECT), is fast and computationally efficient, while exhibiting performance on a par with more complex models in both graph and point cloud classification tasks. Moreover, we show that this seemingly simple statistic provides the same topological expressivity as more complex topological deep learning layers.

==> figures/learn_ect.tex <==

\begin{figure}
  \begin{minipage}[t]{0.47\textwidth}
    \label{fig:learn_ect}
    \center
    \includegraphics[width=0.7\textwidth]{./figures/learn_ect.png}
    \caption{
      The red dots  depict the dataset, a noisy point cloud sampled from a 
      circle.
      The directions are depicted by the grey dots and in the lower left we 
      initialize all angles at the same point. The corresponding ECT in the top 
      left is therefore constant.
      After learning, the directions have spread over the unit circle in the lower 
      right and the ECT matches the ground truth ECT. 
      }
  \end{minipage}\hfill
  \begin{minipage}[t]{0.47\textwidth}
    \label{fig:learn_pointcloud}  
    \center
      \includegraphics[width=\textwidth]{./figures/learn_pointcloud_simple.jpg}
      \caption{Adjust a pointcloud to match another pointcloud using the 
      ECT to compare the point clouds. 
      Both have different number of points and are only matched based on the 
      MSE loss between their ECTs.}
  \end{minipage}
\end{figure}





==> figures/learn_pointcloud.tex <==
\begin{figure}
    \center
    \includegraphics[width=0.5\textwidth]{./figures/learn_pointcloud_simple.jpg}
    \caption{Adjust a pointcloud to match another pointcloud through their 
    ect's. Both pointclouds have different number of points and are only matched
    based on their ECT.}
  \end{figure}

==> tables/all_results.tex <==

\begin{tabular}{llccc}
    \toprule
    Dataset & Type & Model &  Validaton & Test  \\
    \midrule
    \multirow[t]{5}{*}{Manifold} 
     & \multirow[t]{5}{*}{Graph} 
     & ECT + MLP & 1.00 & 1.00  \\
     & & ECT + CNN & 1.00 & 1.00 \\
     & \multirow[t]{5}{*}{Point cloud} 
     & ECT + MLP & 1.00 & 1.00  \\
     & & ECT + CNN & 1.00 & 1.00  \\
    \midrule
    \multirow[t]{5}{*}{CIFAR10} 
     & \multirow[t]{5}{*}{Graph} 
     & ECT + MLP & 0.43 & 0.38 \\
    & & ECT + CNN & 0.51 & 0.49 \\
    & \multirow[t]{5}{*}{Point cloud} 
       & ECT + MLP & 0.42 & 0.42 \\
    &  & ECT + CNN & 0.48 & 0.49 \\
    \multirow[t]{2}{*}{MNIST} 
     & \multirow[t]{2}{*}{Graph} 
        & ECT + CNN & 0.94 & 0.94 \\
     &   & ECT + MLP & 0.65 & 0.69 \\
      & \multirow[t]{2}{*}{Point cloud} 
      & ECT + CNN & 0.95 & 0.94 \\
    &  & ECT + MLP & 0.49 & 0.6 \\  
        \midrule
        \multirow[t]{5}{*}{Modelnet10} 
            & \multirow[t]{6}{*}{100} 
            & ECT + CNN & 0.82 & 0.78 \\
            &  & ECT + MLP & 0.81 & 0.79 \\
            & \multirow[t]{5}{*}{1000}
            &  ECT + MLP & 0.80 & 0.83 \\
            &  & ECT + CNN & 0.87 & 0.84 \\
            & \multirow[t]{5}{*}{5000}
            & ECT + MLP & 0.80 & 0.63 \\
            &  & ECT + CNN & 0.77 & 0.82 \\
            \midrule
        \multirow[t]{4}{*}{Letter-High} 
         & \multirow[t]{4}{*}{Graph} 
            & ECT + CNN & 0.72 & 0.72\\
         &  & ECT + MLP & 0.77 & 0.76 \\
         & \multirow[t]{4}{*}{Point cloud}
            & ECT + CNN & 0.58 & 0.61 \\
         &  & ECT + MLP & 0.47 & 0.52 \\
        \bottomrule
        \end{tabular}
        

==> tables/modelnet.tex <==
\begin{table}[tbp]
    \centering
    \label{tab:modelnet}
    \sisetup{
      detect-all              = true,
      table-format            = 2.2(2),
      separate-uncertainty    = true,
      retain-zero-uncertainty = true,
    }%
    \let\b\bfseries
    \resizebox{\linewidth}{!}{%
      \begin{tabular}{lcSSSSSS}
        \toprule
                        & {100}          &   {1000}  \\
        \midrule
        DeepSets        &  82\pm 2 & 87\pm2 \\
        \midrule
        ECT+CNN (ours)  & 74\pm0.5 &   77.1\pm 0.4 \\
      \end{tabular}%
    }%
    \caption{%
      Results of 5 runs on the 
    }
  \end{table}

==> tables/results.tex <==
\begin{table*}
      \centering
      \setlength{\medmuskip}{0mu}
      \footnotesize
      \sc
      \tabcolsep=3pt
      \begin{tabular}{@{}ccccccccc@{}}
          \toprule
            METHOD      & dd & proteins  \\\midrule
          
            GCN-4        & $72.8\pm4.1$ & $76.1\pm2.4$ \\ 
            GCN-3-TOGL-1 & $73.2\pm4.7$ & $76.0\pm3.9$ \\
            GIN-4        & $70.8\pm3.8$ & $72.3\pm3.3$ \\
            GIN-3-TOGL-1 & $75.2\pm4.2$ & $73.6\pm4.8$ \\ 
            GAT-4        & $71.1\pm3.1$ & $71.3\pm5.4$ \\
            GAT-3-TOGL-1 & $73.7\pm2.9$ & $75.2\pm3.9$ \\ \midrule
            ECT+CNN (ours) & $\b 80.2\pm 2.7$ & $\b76.8\pm 5.4$ \\\bottomrule
          \end{tabular}      
\end{table*}

